FogROS2-Config: Optimizing Latency and Cost for Multi-Cloud Robot Applications

Cloud service providers provide over 50,000 distinct and dynamically changing set of cloud server options. To help roboticists make cost-effective decisions, we present FogROS2-Config, an open toolkit that takes ROS2 nodes as input and automatically runs relevant benchmarks to quickly return a menu of cloud compute services that tradeoff latency and cost. Because it is infeasible to try every hardware configuration, FogROS2-Config quickly samples tests a small set of edge case servers. We evaluate FogROS2-Config on three robotics application tasks: visual SLAM, grasp planning. and motion planning. FogROS2-Config can reduce the cost by up to 20x. By comparing with a Pareto frontier for cost and latency by running the application task on feasible server configurations, we evaluate cost and latency models and confirm that FogROS2-Config selects efficient hardware configurations to balance cost and latency.

==> chapters/design_old.tex <==



\section{\algname}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/system-overview.png}
%     \caption{\textbf{System Overview of \algname} Robot offloads ROS2 nodes through FogROS2 Launcher. The FogROS2 Optimizer finds the best available hardware through optimization, and the runtime application performance in Benchmark Module that dynamically monitors the application latency on cloud. The cloud and robot are connected through FogROS2 Multi-Cloud Connectivity.  
%     }
%     \label{fig:overview} 
% \end{figure}


\algname is a framework that can offload the unmodified ROS2 applications to multiple cloud, and provide fine-grained cost analysis.
It takes a hybrid of system design for multi-cloud robotics and optimization algorithm that automates the analysis of the tradeoff of the latency and cost. 

\begin{listing}[t]
\inputminted[xleftmargin=20pt,linenos,fontsize=\scriptsize,escapeinside=||]{py}{listing/config.py}%
% \begin{tikzpicture}[remember picture, overlay]
%   \node [fit=(pic cs:attrstart)(pic cs:attrend),inner xsep=0.5\linewidth, inner ysep=48pt, xshift=0.5\linewidth, yshift=132pt, rounded corners,draw=black,label={[xshift=70pt, yshift=0pt]State Machine Definition}] {};
%   \node [fit=(pic cs:attrstart)(pic cs:attrend),inner xsep=0.5\linewidth, inner ysep=20pt, xshift=0.5\linewidth, yshift=62pt, rounded corners,draw=black,label={[xshift=70pt, yshift=-15pt]Initial Policy}] {};
% \end{tikzpicture}%
% \vspace{-12pt}
\caption{\textbf{\algname{} Launch Script Example.}  This example launches talker-listener example and offloads talker to the cloud. \algname allows users to directly specify their cost and latency requirement.
Unlike FogROS2 that requires a custom launch description that overrides the standard ROS2 launch description, \algname uses standard ROS2 launch module. The connectivity is implemented as an offloadable ROS2 node to eliminate the complexity of network setup. }
\label{lst:launch}
\end{listing}


% launching process
\subsection{\algname Launcher}
\label{sec:design:launch}
The launching procedure of \algname is inspired by FogROS2~\cite{ichnowski2022fogros}, with an integration of Skypilot that maps hardware type to cloud machine type 
and \algname implements connectivity as an offloadable module to eliminate the complexities of network setup and ROS2 launch system modification.
\algname uses a custom launch extension that is fully integrated with ROS2 launch system. It requires users to identify the ROS nodes to be offloaded to the cloud, but does not need any code changes to the ROS nodes themselves. 
% \eric{highlight features, no modification of ros node, no vpn installation, etc.}

Figure \ref{fig:overview} shows the sequence diagram of \algname.
The following are the steps of \algname launcher that launches the cloud instances:
% \begin{enumerate*}[label=(\arabic*)]
% \item connect to the cloud provider through its programmatic interface to create and start a new instance along with setting up access control to isolate from other cloud computers, and generating secure communication key pairs, 
% \item install the ROS libraries and dependencies on the cloud machine;
% \item copy the serialized ROS nodes and ROS workspace from the robot to the cloud machine;
% \item (optional) launch constainerized ROS nodes;
% \item launch offloaded ROS nodes;
% \end{enumerate*}
(1) User provides the ROS2 nodes that need to be offloaded to the cloud, and specifies the latency and per-request cost constraints of the ROS2 nodes;  
(2) FogROS2-Sky Optimizer finds the  cost-effective hardware that fulfills the constraints by 
    (2.A) sampling from the hardware specification, 
    (2.B) conduct benchmark on the hardware specification 
    (2.C) Modeling the Latency 
    (2.D) Modeling the Cost function, 
    (2.E) Find the optimal of the latency and cost function that fulfills the constraints; 
(3) Use Skypilot to launch and manage multi-cloud virtual machines 
(4) Provision the multi-cloud virtual machines by setting up the ROS2 environment and workspace 
(5) Setup the benchmark module for monitoring the latency and cost performance of the application 
(6) Launches the application ROS2 nodes on the cloud 
(7) Launches FogROS2-Multi-Cloud Connectivity to securely and globally connect the robot with the multi-cloud virtual machines
At the same time, the ROS2 launch system initiates ROS nodes on the robot.


% cost 
\subsection{Fine-grained Cost Analysis}
\algname enables fine-grained cloud robotics cost analysis by simultaneously benchmarking on multiple cloud machines and dynamically collect the timing from ROS2 applications. One can specify potential candidates such as hardware requirement (number of CPU, type of GPU) or cloud machine type specific to the cloud service providers. 
% command line integration \eric{todo in code!! what's the interface for doing the benchmark related analysis} 
The ROS2 timing is collected from the callback of the ROS2 applications 
such as per neural network inference. 

\textbf{ROS2 latency collection}
% Users can choose from two approaches that can collect latency (1)  (2) We acknowledge that it is hard to modify the inheritance of some applications. 
\algname runs a sidecar process that passively collects the request and response ROS topics, and uses the difference between the response message and request message to determine the latency. Alternatively, users can use \algname callback at the start and end of the desired latency collection period that requires three line modification in the application code. 
The collected latency statistics are written to a file that can be collected by the robot. 

\textbf{Latency-to-Cost Calculation}
Once the benchmark condition is fulfilled, such as when the set time has elapsed or the requisite number of latency statistics is collected, \algname orchestrates the files from all the candidates and queries Skypilot~\cite{}  interface for the cost of the cloud machine.
\algname utilizes the hourly rate information gathered from Skypilot to calculate the cost of using a machine for a single second. The total cost for a specific ROS2 request is determined by multiplying this per-second cost by the number of seconds required to complete the request.

% network 
\subsection{Secure Multi Cloud Connectivity}
% Sky cannot do it 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/sgc_comparison.png}
    \caption{\textbf{Connectivity Mechanism Difference of \algname and FogROS2-SGC}(a) FogROS2-SGC connects ROS nodes across different domains by using intermediate routers (b) \algname uses a signaling registry server that facilitate propagating the routing information, instead of the data itself, and the actual data is sent directly between ROS nodes. This reduces the transmission latency of the data.} %This reduces the coordination protocol overhead and eliminating the intermediate routing hops also improves the network latency by \eric{show numbers}}
    \label{fig:sgc_comparison}
\end{figure}

% webrtc and how the protocols are decomposed 
\algname facilitates the connection of distributed ROS2 nodes on robots and cloud, making them operate as if they are on the same machine. The connectivity of ROS2 nodes can be scaled across multiple cloud data centers in various geographic locations
Existing connectivity solutions fall short in this context: FogROS2 needs manual VPN setup;  Skypilot's use of reliable object storage is incompatible with ROS2's publish-subscribe communication; the unnecessary peer-to-peer assumption in FogROS2-SGC's routing infrastructure leads to increased latency since cloud servers are already mutually accessible.

\algname enables ROS2's multiple-party publish-subscribe communication model by extending the capacity of the DataChannel in webRTC, that allows direct peer-to-peer bidirectional communication, which is usually used in browser-based file transfer or real-time text communication. 
The original DataChannel is designed to support only two peers, and all connections must initiate in a specific sequence that channel opener must start before joiner can join. In contrast, multiple-party publish-subscribe in ROS2 requires $m$ publishers to mutually connect with $n$ subscribers with $O(mn)$ connections, and these publishers and subscribers can start in any order. 

% multiple part ypub/sub
To resolve this issue, \algname uses a \emph{callback-based signaling registry} to facilitate multiple-party publish-subscribe on DataChannel. The registry only facilitates to build the connection between nodes, making it lightweight and hostable at any known network address to which both the robot and cloud servers can connect.
The registry doesn't route any actual data and is not on the critical path of actual application performance. 

In this approach, ROS2 publishers and subscribers of the same topic are registered in the registry. All ROS publishers also register a callback such that when there is a new subscriber to the topic, the publisher creates a unique DataChannel for that publisher and subscriber. ROS2 subscribers register a callback triggered when the unique DataChannel is created. If the publisher's DataChannel is created, the subscriber can join the unique DataChannel and communicate with the publisher through it. Both publishers and subscribers continually listen to the callback in case new publishers and subscribers register with the registry.

% concluding results and discussions
Figure \ref{fig:sgc_comparison} illustrates the mechanism difference between webRTC, FogROS2-SGC and \algname. Both FogROS2-SGC and \algname uses DTLS protocol\cite{dtls_algorithm} as the underlying data transport for both low latency transmission and security, so the actual data delivery latency is similar, but \algname uses less routing hops compared to FogROS2-SGC.
In some rare cases, having intermediate routers may perform better if the source publisher has bandwidth limitation and need to broadcast to multiple subscribers, but \algname also supports the peer-to-peer relationship as FogROS2-SGC, so the publisher is connected with an intermediate routing node with higher bandwidth, which facilitates the routing to other subscribers.

% \eric{this part is not necessary (?)}
% We recognize that robots are usually run under CPU processing constraints, and packet processing (including network operation, encryption) should have minimal interference with the actual application computation. \algname significantly reduces the CPU usage from \sgc. In \sgc, its proxy creates a ROS node thread for every ROS topic, and busily spins even if no topic is created. This approach is responsive to new messages and reduces the critical path of the message processing, but it wastes significant CPU cycles and affect the application performance of the actual applications. In addition, ROS2 node creation is not thread-safe~\cite{}, which leads to software instability or crashing if multiple nodes are created concurrently. 

% In \algname, we orchestrate all the ROS topic management into one topic management thread, which we use a shared and mutex-guarded data structure to manage the addition and reduction of the new topics. The data structure stores the mapping from topic name to topic state (actively publish, actively subscribe, paused, deleted) and the list of the receiver threads (network connections) of other remote publishers or subscribers. All the messages need to first go through the topic management thread to be forwarded to the actual destination thread (network thread or ROS2 thread). This helps with controlling and reconfiguring the forwarding states of the ROS2 topic.


\subsection{Connectivity as an offloadable module}
\eric{given we are running out of space, im planning to combine this with the previous section}
\algname uses a proxy-based design for multi-cloud connectivity. It serves as a bidirectional interface between the global multi-cloud connectivity network and the local ROS2 network. 
Users specify desired ROS2 topics to publish or subscribe to via a configuration file. In response, the proxy initiates a local ROS2 publisher or subscriber for each topic. Messages from the local ROS2 network are captured by the proxy and forwarded to the \algname network. Upon receipt, verified subscribers convert these messages into standard ROS messages and publish them on their local ROS2 networks. 

As shown in Listing \ref{lst:launch}, the proxy is encapsulated as a typical ROS2 node that can be offloaded to the cloud, thus compatible with the standard ROS2 launch system. This facilitates its cloud-based offloading alongside \algname, eliminating the need for VPN or DDS-specific configurations to achieve distributed ROS node connectivity.



==> chapters/evaluation_v1.tex <==
\section{Evaluation}

We use an Intel NUC with an Intel\textsuperscript\textregistered{} Pentium\textsuperscript\textregistered{} Silver J5005 CPU @ 1.50\,GHz to act as the robot. 
We perform most evaluations with cloud nodes deployed to AWS and partially on Azure if specified.  

\subsection{Optimization}
We note that the price of the cloud service provider changes hourly, so all the experiments need to be conducted at the same time for fair comparison. The experiment results shown are conducted at Sept 2023. We choose XXX, XXX, XXX as the latency and cost bound for the three applications, and later we show that the bound selection does not affect the accuracy of the \algname optimizer. 

We compare against the following baseline models: (1) \textbf{Full Benchmark}:  We run the benchmark code out of all the available CPU cores with the associated default memory size \eric{what do we do here?}. The exhaustive search can find the optimal one within a given hardware family, which serves as ground-truth for our optimization algorithm. The optimal machine is selected as the machine closest to the user defined constraint.
In Visual SLAM experiment, we cap CPU cores to be less than 64 cores, since we know that it is less computationally heavy compared to other algorithms. (2) \textbf{Iterative Binary Search} We select iterative binary search as an empirical approach that iteratively finds the closer binary partition to user's constraint. 
We note that both baselines only work with the change of one variable. Changing two variables (memory and CPU cores) at the same time is prohibitive due to the cost and time limitation. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/benchmark_table.png}
%     \caption{\textbf{Evaluation of \algname optimizer} on vSLAM, Motion Planning and grasp planning for finding optimal hardware specification. \algname is X times, X times and X times faster, and X times cheaper.}
%     \label{tab:benchmark_table}
% \end{figure}


Table \ref{tab} shows a comparison of \algname with other baselines in finding the optimal hardware specification in the cost and time needed to converge to a solution, and the optimality of the final result. From the experiments, we show that 
 \algname is X times, X times and X times faster, and X times cheaper...
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/optimization_fitting.png}
    \caption{\textbf{Comparison of \algname estimation and the ground-truth} The dotted are actually benchmarked and lines are estimated by the optimizer based on the benchmark results. \algname results in the same estimation at the constraint point. }
    \label{fig:optimization:fitting}
\end{figure}

Figure \ref{fig:optimization:fitting} shows the estimation of \algname optimizer with the ground truth in both the time and cost function.

\textbf{Handling Failures and Dynamism} We study the behavior how user defined bound can affect the . 

\subsection{Connectivity}
We compare the message round trip latency of multi-cloud connectivity in \algname with VPN used in FogROS2 and FogROS2-SGC with one intermediate routing hop. We use a separate Azure cloud machine as the router of FogROS2-SGC at California, so that the router is geographically close to the robot, cloud machine. Figure \ref{fig:eval:latency} shows the latency of \algname. 

\subsection{Dex-Net Case Study}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/gqcnn_setting_2.png}
    \caption{\textbf{Grasp Planning with Dex-Net}
    A robot (left) with an attached computer (e.g., an Intel NUC) sends RGBD image observations from an overhead camera (middle) to compute grasps using a Dex-Net Grasp Quality Convolutional Neural Network (GQCNN) on a cloud computer with a GPU.  The result (right) is grasps poses (green) and their relative quality score (q-value) for parallel-jaw (top-right) and suction gripper (bottom-right). \eric{text from fogros2 paper}
    }
    \label{fig:dex-net_example}
\end{figure}

In this section, we perform a cost analysis study of grasp planning framework in ROS2, Dex-Net with \algname. 
Dex-Net~\cite{mahler2017dex} uses a deep neural network to compute grasp contact points given a depth image.  This allows a robot to determine the grasp that is most likely to succeed when picking up an object. FogROS~\cite{chen2021fogros} suggests using GPU hardware accelerator can significantly improve the latency, so we choose four candidates with two major cloud service providers and three most popular GPU types, respectively T4 on AWS, K80 on Azure, M60 on AWS and an 8-core CPU only baseline. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{image/misconception.png}
    \caption{A comparison of cloud robotics cost across different cloud service providers and hardware accelerator types on Dex-Net. }
    \label{fig:dexnet-benchmark}
\end{figure}

Figure \ref{fig:dexnet-benchmark} shows the benchmark results collected at April 3, 2023 with 100 Dex-Net requests. We observed that Azure's K80 offers similar request latency (4.2 seconds) but the price is 2.5x compared to using a pure CPU-only machine on AWS. Due to the account limitation, we are unable to benchmark other GPU options on Azure. Additionally, even within the same provider AWS, both M60 and T4 are popular GPU acceleration choices and get similar performance, but M60's per-request cost is 2.3 times higher than T4. 

The observation leads to a conclusion that \textbf{higher spending on cloud service providers does not necessarily yield better application performance}. Even if knowing hardware candidates, one has to benchmark their applications to find the best available cloud machine that fulfils the application requirement. 

==> chapters/optimization_v1.tex <==
\section{\algname Sampler}





\subsection{FogROS2-Sky Optimization}

% In the previous section, we discuss how FogROS2-Sky extends the Sky framework for robotics applications \cite{chasins_sky_2022}. It creates the most cost-effective cloud instance to complete a task while considering financial, time, and resource constraints. However, 
% selecting optimal hardware resources for a task without extensive cloud computing knowledge can be challenging. More expensive resources do not always guarantee better performance, which can make it difficult to find the best hardware.

% To improve accessibility for individuals without cloud experience, this paper also proposes a preliminary optimization step to select the most suitable hardware resources based on financial and temporal constraints. 
With \algname,  users need only input the task, step count, time, and cost, and the optimizer determines the required resources. The task refers to an algorithm (i.e. Dexnet, ORB-SLAM, etc.) and its corresponding ROS2 setup configuration and launch file. The step count refers to the number of iterations the user wants to run in the algorithm. With these components, the best-case hardware is calculated and inputted into FogROS2-Sky to find the best cloud instance. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/optimizer_sky.png}
%     \caption{Overall FogROS2-Sky Pipeline with Optimizer.}
%     \label{fig:sky_optimization}
% \end{figure}

The overall goal of this optimization problem is to identify cloud resources (CPU count, GPU type, and memory) that best align with a given task while adhering to cost and time constraints. While we could develop a loss function to try to effectively balance time and cost, every user has their own preferences on how time and cost should be weighted for a given task. Instead, we divide the problem into two parts: minimizing financial cost and minimizing time. Users are then presented with both results and can choose the option that best suits their needs. 

We formulate it as an optimization problem of minimizing the latency per request $time(x)$ and financial cost per request $cost(x)$ with hardware specification $x = \{x_1, x_2\}$ , where $x_1$ is the CPU core count and $x_2$ is the memory size in GB. 
% \charlotte {maybe replace: "...$x = \{x_1, x_2\}$, where $x_1$ is the CPU core count and $x_2$ is the memory size in GB."}
Our optimization problem is formulated as following: 
% \begin{figure}
% \centering
% \textbf{Optimization Setup}
% \medskip

{\small
\textbf{Objective Function:}
\begin{align*}
    \alpha \cdot \text{time}(x) + \beta \cdot \text{cost}(x)
\end{align*}

% \textbf{With Constraints:}
% \begin{align*}
%     x_1 &\geq \text{Max CPU} \\
%     x_1 &\leq \text{Min CPU} \\
%     x_2 &\geq \text{Max Memory} \\
%     x_2 &\leq \text{Min Memory} \\
%     \frac{x_2}{x_1} &\geq \text{Max Memory:CPU} \\
%     \frac{x_2}{x_1} &\leq \text{Min Memory:CPU} \\
%     \text{time}(x) &\leq \text{Max Time} \\
%     \text{cost}(x) &\leq \text{Max Time}
% \end{align*}
\textbf{With System Constraints:}
\begin{align*}
    x_1 &\geq \text{Max CPU} & x_1 &\leq \text{Min CPU} \\
    x_2 &\geq \text{Max Memory} & x_2 &\leq \text{Min Memory} \\
    \frac{x_2}{x_1} &\geq \text{Max Memory:CPU} & \frac{x_2}{x_1} &\leq \text{Min Memory:CPU}
\end{align*}
% \vspace{-1em}

\textbf{With User Constraints:}
\begin{align*}
    \text{time}(x) &\leq \text{Max Time} \\
    \text{cost}(x) &\leq \text{Max Cost}
\end{align*}
% \begin{equation*}
%     \text{time}(x) \leq \text{Max Time}
% \end{equation*}
% \begin{equation*}
%     \text{cost}(x) \leq \text{Max Time}
% \end{equation*}
}

We run the two forms of this optimization: one where $\alpha = 0$ and $\beta = 1$ for cost optimization and one where $\beta = 0$ and $\alpha = 1$ for time optimization. 


In future work, users can input their desired weighting of cost and time to further tailor the optimization for their needs.

CPU count and memory are treated as primary variables since they are continuous. 
% We solve this problem using SciPy's optimization library. 
However, it is important to note that CPU count and memory are not truly continuous values as it is impossible to have a float CPU or memory count (i.e.  (6.72 CPU, 2.84 GB)) and it is inefficient to have an unspecified CPU or memory count (i.e (7 CPU, 3 GB) when the only available machines are (4 CPU, 2 GB) and (8 CPU, 4GB). Therefore, the optimizer works in continuous space and creates a solution subset by rounding to the nearest feasible options and selects the optimal solution from the subset that best minimizes loss and satisfies constraints.

The GPU type introduces an additional challenge due to its discrete nature. To address this issue, the optimizer will fit a custom time and cost function to each GPU type and solve separate optimization problems. The results from these problems are then compared with each other, and the program returns the hardware configurations that meet the constraints and best minimize the loss function.

% \caption{FogROS2 Sky Optimization Framework. As described earlier, }
% \label{fig:optimization_framework}
% \end{figure}



% \begin{figure}[h]
%     \centering
%     \caption{FogROS2 Sky Optimization Framework (top) Time Optimization (bottom) Cost Optimization. We specify arbitrary values for minimum memory and CPU count as opposed to 0 because cloud service providers also have arbitrary hardware minimums. This improves the optimizer's efficacy as it ensures the outputs specify the hardware requirements for a feasible cloud instance.}
%     \label{fig:optimization_framework}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{image/optimization_flowchart.png}
%     \caption{FogROS2 Optimizer Flowchart.}
%     \label{fig:optimization_flowchart}
% \end{figure}



The FogROS2-Sky optimizer relies on being able to determine time and cost as a function of hardware. Since there is no intuitive understanding of how time and cost relate to hardware, we employ sky benchmarking to fit functions for these parameters. Benchmarking leverages multithreading for parallel processing to significantly speed up the optimizer. Specifically, we simultaneously sample various hardware configurations and run them for 5 minutes to determine seconds per step and dollars per second as outlined in Table \ref{tab:opt:sample}. We chose to only benchmark for 5 minutes to minimize the time and cost of hardware sampling. 

\input{table/data_sample}

Since the user inputs the desired number of algorithm steps, we can use the benchmarking data to create time and cost functions. These functions take the form of either constant, linear, hyperbolic, power, log, or exponential regression based on best fit with respect to the determination coefficient $R^2$. We chose regression-based models opposed to Gaussian Processes or Neural Networks to mitigate the risk of overfitting since we only sample a few hardware combinations. Finally, we frame the optimization problem using these functions and use SciPy's optimization library to identify the optimal hardware solution.

\textbf{Dynamic Constraint Adjustment} \algname optimizer supports changing the constraints without re-running the benchmark. 
The users can tune their cost and performance tradeoff by directly applying the constraints on the cost and latency models, without re-running the benchmarks. 
When launching the actual ROS2 applications at the deployment, \algname first checks if the saved cost and latency function exist, and initiate the cloud machines from the earlier generated models.
% \eric{TODO: how does the algorithm adjust the price changes? or does it? }

\subsection{Secure Multi Cloud Connectivity}
\algname uses a proxy-based design for multi-cloud connectivity with FogROS2-SGC~\cite{chen_fogros2-sgc_2023}. It serves as a bidirectional interface between the global multi-cloud connectivity network and the local ROS2 network. 
Messages from the local ROS2 network are captured by the proxy and forwarded to the \algname network. Upon receipt, verified subscribers convert these messages into standard ROS messages and publish them on their local ROS2 networks. 
We encapsulate the proxy into a typical ROS2 node that can be offloaded to the cloud, thus compatible with the standard ROS2 launch system (Listing \ref{lst:launch}). This facilitates its cloud-based offloading alongside \algname, eliminating the need for VPN or DDS-specific configurations to achieve distributed ROS node connectivity.

